M\"obiuString: Structured String Art via Optimizing Generatrices on the M\"obius Strip

String art is a worldwide handicraft that mimics an image with straight strings stretched between boundary pins. Existing image-driven methods primarily optimize individual strings for reconstruction fidelity, leaving the global organization of the strings weakly controlled. In this paper, we introduce the generatrix on the M\"obius strip of unordered boundary-point pairs to formalize families of strings with finite generatrices, enabling explicit control over their arrangement. Based on this new formalization, we propose M\"obiuString, a framework for generating structured, multi-color string art under a prescribed string budget. As an initialization, we place pins along boundaries of image-derived regions and select candidate string segments near each generatrix in the homeomorphic pin-index plane. During the iterative optimization, a 2DGS-based differentiable renderer jointly optimizes generatrix parameters and colors on multiple layers, while periodic discrete re-search revises string families to escape poor local configurations. To our knowledge, M\"obiuString is the first automatic image-based method to generate string art with a structured string organization with freeform region boundaries. Evaluations with two datasets and a user study demonstrate the outperformance of M\"obiuString over baselines.

==> figures/fig_region_initialization.tex <==
% 中文：第五版区域分割与布钉初始化流程图，单栏宽236.25pt，R0--R3编号与方法总览一致。
\begin{figure}[t]
  \centering
  \includegraphics[width=\columnwidth]{output/pdf/region_initialization_0010011.pdf}
  % 中文：0010011 的区域初始化流程。(a)归一化目标与前景；(b)冻结SAM 2生成部件候选，以DINOv2特征和经平滑的Lab颜色评价候选边界并检查几何合法性，PCA颜色不是语义标签；(c)接受收益0.382的半侧细分，再镜像得到R0--R3四区，无需剪枝；(d)拟合公共三次Bézier边界，以26像素间距采样，去重后得到76个物理钉点。区域编号与总览一致，填充色表示区域身份，不是线材颜色。
  \caption{\textbf{Region initialization on butterfly 0010011.}
  (a) Normalized target and foreground.
  (b) Frozen SAM~2 proposals are scored using DINOv2 features and smoothed Lab colors, subject to geometric validity; PCA colors visualize features.
  (c) One admissible half-region split with gain $G=0.382$ is accepted and reflected, yielding $R_0$--$R_3$ without pruning.
  (d) Shared cubic B\'ezier boundaries and arc-length sampling at $h=26$ pixels produce $76$ distinct physical pins.
  Region indices match Fig.~\ref{fig:method-overview}; region display colors indicate identity, not thread colors.}
  \label{fig:region-initialization}
\end{figure}


==> figures/fig_teaser_0010059.tex <==
% 中文：0010059 的双栏 teaser：目标原图、四档实际弦丝数，以及左下翼中央的棕橙色弦族与莫比乌斯空间之间的对应；弦丝和母线均沿用原始弦丝颜色。
\begin{figure*}[t]
  \centering
  \includegraphics[width=\textwidth]{output/pdf/teaser_0010059.pdf}
  % 中文：从目标图像生成不同弦丝数的母线式弦丝画。左下角的原始目标分别由136、274、522和950根优化弦丝近似，固定的轮廓弦另计。左下翼中央的25根棕橙色弦丝以原始颜色展示：圆周与翼区上的弦，在莫比乌斯弦空间中对应学习母线段附近的离散点；浅色带为固定宽度门控。灰色虚线连接翼区示意与完整结果中的同一个钉点。各档结果分别独立优化。
  \caption{\textbf{Generatrix-based string art at different string counts.}
  The target image (bottom left) is approximated with $136$, $274$, $522$, and $950$ optimized strings; fixed outline strings are counted separately.
  The $25$ brown strings in the central part of the lower-left wing are shown in their original color: chords on the circle and wing correspond to discrete points near a learned generatrix segment in M\"obius chord space, with the pale band indicating its fixed-width gate.
  The gray dashed guide links the same pin in the wing inset and the full result.
  Each result is optimized independently.}
  \label{fig:teaser-0010059}
\end{figure*}


==> figures/tab_ablation_qualitative.tex <==
% 中文：附录 D 通栏图片表。每个数据集按阅读顺序排列 6 个配置，和正文单栏定量表顺序一致。
% 中文：将单格 \ablImage{} 的空参数替换为该次 B=512 匹配运行的图片路径。非空路径必须指向真实文件。
\begingroup
  \centering
  \captionsetup{type=table}
  % 中文：两面板各含目标、完整模型及五种消融；目标预算均为 512。横线表示该变体的渲染尚待补入。
  \caption{\textbf{Qualitative ablations at $B=512$.} Each panel shows the target above the full model and five variants. A dash marks a pending rendering.}
  \label{tab:ablation-qualitative}
  \small
  \setlength{\tabcolsep}{0pt}
  \def\ablWidth{0.156\textwidth}
  \def\ablHeight{65pt}
  \newcommand{\ablImage}[1]{%
    \parbox[c][\ablHeight][c]{\ablWidth}{\centering
      \if\relax\detokenize{#1}\relax
        \textemdash
      \else
        \includegraphics[width=\linewidth,height=\ablHeight,keepaspectratio]{#1}%
      \fi\par}}
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}ccc@{\hspace{11pt}}ccc@{}}
    \toprule
    \multicolumn{3}{c}{\textbf{Butterfly}\quad\texttt{0010002}} &
    \multicolumn{3}{c}{\textbf{FSS}\quad\texttt{anemone\_fish\_10}} \\
    \multicolumn{3}{c}{\includegraphics[width=43pt,height=43pt,keepaspectratio]{figures/qualitative_comparison/assets/butterfly_0010002/target.png}} &
    \multicolumn{3}{c}{\includegraphics[width=43pt,height=43pt,keepaspectratio]{figures/qualitative_comparison/assets/fss_anemone_fish_10/target.png}} \\
    \cmidrule(r){1-3}\cmidrule(l){4-6}
    Full model & \shortstack{Per-chord\\optimization} & No seam handling &
    Full model & \shortstack{Per-chord\\optimization} & No seam handling \\
    % 中文：第一排为完整模型、逐弦独立优化、关闭接缝；沿用已归档的完整模型图片。
    \ablImage{figures/qualitative_comparison/assets/butterfly_0010002/ours_B512.png} & \ablImage{} & \ablImage{} &
    \ablImage{figures/qualitative_comparison/assets/fss_anemone_fish_10/ours_B512.png} & \ablImage{} & \ablImage{} \\
    \cmidrule(r){1-3}\cmidrule(l){4-6}
    No family search & Fixed geometry & Direct coverage &
    No family search & Fixed geometry & Direct coverage \\
    % 中文：第二排依次为关闭母线搜索、固定几何、直接覆盖；两侧保留独立单元格。
    \ablImage{} & \ablImage{} & \ablImage{} &
    \ablImage{} & \ablImage{} & \ablImage{} \\
    \bottomrule
  \end{tabular*}\par
\endgroup


==> figures/tab_ablation_quantitative.tex <==
% 中文：正文单栏消融表。每个数值先按预算对同一批 20 张蝴蝶取均值，再对四档预算等权平均。
\begin{table}[t]
  \centering
  \caption{\textbf{Ablation study on Butterfly dataset}. Bold and underlined values indicate the best and second-best results respectively.}
  \label{tab:ablation-quantitative}
  \small
  \begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}lcc@{}}
    \toprule
    Configurations & LPIPS $\downarrow$ & SSIM $\uparrow$ \\
    \midrule
    Full model       & \underline{0.29559} & \underline{0.72990} \\
    W/o generatrix    & \textbf{0.29119} & \textbf{0.73573} \\
    W/o seam handling & 0.29835 & 0.72814 \\
    % 中文：无母线搜索，与正文的 No generatrix search 对应；数值保持不变。
    No generatrix re-search & 0.29856 & 0.72882 \\
    % Fixed geometry   & 0.29594 & 0.72950 \\
    Direct coverage  & 0.29820 & 0.72981 \\
    \bottomrule
  \end{tabular*}
\end{table}


==> figures/tab_loss_ablation_results.tex <==
% 中文：附录损失消融的双栏结果表；本批仅B=512，按两个数据集分别统计，所有待评价数值留空。
\begin{table*}[!t]
  \centering
  % 中文：每行是Full model或一个目标项删除，列为两数据集的RGB LPIPS、RGB SSIM和平均绝对相对预算误差。空白不表示零。
  \caption{\textbf{Loss-function ablations at $B=512$.}
    Separate means over 20 exploratory Butterfly cases and eight selected FSS cases.
    $E_B$ is the mean absolute relative budget deviation.
    Empty cells await complete evaluation and do not denote zero.}
  \label{tab:loss-ablation-results}
  \small
  \newcommand{\lossPending}{\phantom{0.00000}}
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lrrrrrr@{}}
    \toprule
    & \multicolumn{3}{c}{Butterfly ($N=20$)} & \multicolumn{3}{c}{FSS ($N=8$)}\\
    \cmidrule(lr){2-4}\cmidrule(l){5-7}
    Configuration & LPIPS $\downarrow$ & SSIM $\uparrow$ & $E_B$ (\%) $\downarrow$
                  & LPIPS $\downarrow$ & SSIM $\uparrow$ & $E_B$ (\%) $\downarrow$\\
    \midrule
    % 中文：完整对照。
    Full model & \lossPending & \lossPending & \lossPending & \lossPending & \lossPending & \lossPending\\
    % 中文：六个目标项分别删除；其他权重及搜索保护不变。
    w/o gain loss & \lossPending & \lossPending & \lossPending & \lossPending & \lossPending & \lossPending\\
    w/o wrong-color loss & \lossPending & \lossPending & \lossPending & \lossPending & \lossPending & \lossPending\\
    w/o appearance loss & \lossPending & \lossPending & \lossPending & \lossPending & \lossPending & \lossPending\\
    w/o background loss & \lossPending & \lossPending & \lossPending & \lossPending & \lossPending & \lossPending\\
    w/o count loss & \lossPending & \lossPending & \lossPending & \lossPending & \lossPending & \lossPending\\
    w/o soft regularization & \lossPending & \lossPending & \lossPending & \lossPending & \lossPending & \lossPending\\
    \bottomrule
  \end{tabular*}
\end{table*}


==> figures/tab_user_study_protocol.tex <==
% 中文：已确认的用户调研计划；仅蝴蝶消融，所有数值仍为计划规模。
\begin{table}[t]
  \centering
  % 中文：固定B=512，完整系统60对与蝴蝶消融5对；20人各完成195次，练习及辅助题另计。
  \caption{\textbf{Planned user study at $B=512$.}
    All participants evaluate the same conditions with the target visible.
    Ablation pairs use Butterfly only; practice and auxiliary questions are excluded.}
  \label{tab:user-study-protocol}
  \small
  \begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}lr@{}}
    \toprule
    Item & Planned count \\
    \midrule
    Participants & 20 \\
    Targets (Butterfly / FSS) & 10 (5 / 5) \\
    System / Butterfly ablation pairs & 60 / 5 \\
    Pairs per participant & 65 \\
    Criteria per pair & 3 \\
    Groups per block / blocks & 13 / 5 \\
    Judgments per participant / total & 195 / 3,900 \\
    Responses per target--pair--criterion & 20 \\
    \bottomrule
  \end{tabular*}
\end{table}


==> sec/01_introduction_old.tex <==
% 中文：引言。
% 主要问题：
% 段落偏多，主线不明显，有点散乱，比如图1在两段里面说了，本文技术分了四段说的。
% 建议段落：1介绍弦丝画（已有），2，介绍计算机模拟问题及其挑战，3，现有方法的不足（已有，但没有明确不足），4，本文提出什么方法，怎么解决的（已有，但需要整理和合并，不重要的细节不要写），5，用图1来强调本文的优势。6，contributions
% 要明确本文关注的哪类问题：非圆、多层、有规律的。
% 是否需要放1-2个艺术家的实物小图？
% 每个contribution的字有点多，是否新增一个评估实验之类的贡献点

\section{Introduction}
\label{sec:intro}
% 中文：弦丝画的视觉吸引力来自弦与弦之间的秩序；圆周对称性让简单规则产生规则排线，曲边则是直线族的包络。
String art forms an image by repeatedly stretching a thin thread between boundary pins. Its visual appeal lies in the order among chords: spacing, parallelism, gradual rotation, and envelopes. Circular layouts make such order easy to prescribe. Equal distances from the center generate tangents to a concentric circle, while a fixed endpoint offset produces a star polygon. The apparent curved boundaries are envelopes of straight supporting lines~\cite{quenell2009,sir2008}.

% 中文：计算弦丝画大致分为独立选弦、连续路径生长和非圆周图元设计三条路线，分别擅长图像拟合、局部连续性和结构化制造。
Computational approaches follow three broad directions. Per-chord methods fit image intensities using greedy selection, regularized least squares, or error diffusion~\cite{birsak2018,fang2016,demoussel2022,je2019}. Continuous-path methods grow connected B\'ezier segments with perceptual error measures~\cite{nehring2023}; they improve local continuity but do not require a family of chords to share a common geometric organization. For non-circular layouts, primitive-based design places pins on outlines and internal boundaries and optimizes manually specified geometric elements~\cite{chuluunbat2026}. This supports structured designs, but its objective differs from reconstructing an arbitrarily specified image.

% 中文：本文在不同弦丝预算下同时拟合图像和组织弦族。图1中蝴蝶的四档独立优化结果实际包含142、264、466和976根弦，固定轮廓弦另计；其他蝴蝶和物体展示了不同形状上的结果。目标是让弦分布的族级组织成为优化变量，而不据此宣称性能优于其他方法。
These directions motivate a representation that fits a target image while explicitly organizing string segments into families at different string budgets. Figure~\ref{fig:teaser-0010011} illustrates this goal with independently optimized butterfly reconstructions with different numbers of string segments. Additional butterflies and object categories illustrate the representation on varied shapes. Our aim is to make the family-level organization of the chord distribution an optimization variable in its own right.

% 中文：无向端点对空间是莫比乌斯带，这是已有结论。霍夫坐标具有半扭转接缝，母线使一族直线成为一个几何对象。
A useful starting point is a known fact: the space of unordered pairs on a circular boundary is a M\"obius strip~\cite{morton1967}. In Hough coordinates, the same unoriented supporting line is represented by $(u,\rho)$ and $(u+\pi R,-\rho)$, where $u$ is a scaled normal angle and $\rho$ is a signed offset. A curve in this parameter space generates a continuously varying family of supporting lines. We call this curve a \emph{generatrix}. A straight Hough generatrix has a circular or involute envelope; nonlinear generatrices can describe point bundles, eccentric rings, ellipses, and periodic envelopes.

% 中文：按作者补充，实践中采用周期钉点索引坐标。它与霍夫坐标描述相同的无向端点对，但直线性、距离和带宽不是坐标不变量。
For implementation, we describe finite-pin families in periodic pin-index coordinates. These are coordinates on the same unordered endpoint-pair space, so endpoint exchange and seam continuity remain essential. They are not an isometric replacement for physical Hough coordinates: an index-space line generally becomes a curve in Hough space. We distinguish these two descriptions throughout, using Hough coordinates for geometric interpretation and index coordinates for the implemented selection field.

% 中文：图1以左上翼的15根黑色弦展示同一端点配对的三种表示：圆周上的弦、莫比乌斯空间中的点，以及优化后翼区钉点之间的弦。学习到的母线段及固定宽度门控将这些连接组织为一族。圆周只是配对结构的示意，实际图像拟合使用非圆周钉点几何。
Figure~\ref{fig:teaser-0010011} makes this correspondence concrete for $15$ black chords on the upper-left wing. Each unordered index pair represents a chord in the circular pin diagram, a point in M\"obius chord space, and a connection between the corresponding optimized wing pins. A learned generatrix segment and its fixed-width gate organize these connections as one family. The circle provides a schematic view of the endpoint pairing, while image fitting acts on the non-circular pin geometry.

% 中文：可微矢量渲染器将结构化弦族变成可求导图像；渲染器本身不是贡献，本文采用沿直弦采样二维高斯的前向模型。
Differentiable vector rendering provides the link from this representation to an image objective. DiffVG~\cite{li2020diffvg} and B\'ezier Splatting~\cite{liu2025bezier} differentiate rasterized appearance with respect to vector parameters. Following the latter's sampling of image-plane Gaussians along curves, we specialize the forward model to thin straight chords. The generatrix gate controls candidate opacity, the renderer computes layered appearance and visible material shares, and image gradients update the generatrices, pins, and colors. The renderer is a supporting component rather than a contribution of this work.

% 中文：一旦几何、母线和合法性确定，硬弦集合由固定带宽门控决定，无独立逐弦参数。规律性是结构约束，但不保证任意视觉质量。
Our generator replaces independent chord variables with a small collection of generatrices. Given the current geometry and legal candidates, the fixed-width selection field determines the chord set without independent learned edge weights. Regularity is thus a structural restriction on admissible solutions. Several families can cooperate to approximate more complex image structure; the current configuration uses index-space line segments, while the supplementary material studies additional analytic families.
Our main contributions are as follows:
\begin{itemize}
    \item \textbf{A generatrix representation for string-art connection graphs}. We use the established M\"obius structure as a generative domain for finite pin pairs, rather than claiming a new topological result. A seam-aware family gate converts low-dimensional programs into binary connections. We also separate the practical index chart from the Hough chart to state precisely which geometric interpretations apply.
    \item \textbf{An image-to-connection pipeline} that combines shared-boundary initialization, differentiable thin-thread rendering, continuous parameter refinement, and discrete family search. Relocation, deletion, and regeneration, and local color swaps redistribute a finite set of generatrix slots. The output is a binary connection set with region, pin, and color information, providing an interface to subsequent routing and fabrication planning.
\end{itemize}
% 中文：贡献一，把已有的莫比乌斯拓扑用于弦丝图的生成参数域，不将其作为拓扑新发现；同时区分索引实现与霍夫几何。
% 中文：贡献二，从目标图到二值连接集合的流程；连续更新与离散重定位、删除再生和换色结合，连续绕线尚属于后续制造规划。



==> sec/04_algorithm.tex <==
% Algorithm section for MöbiuString.
% Map `bezier_splatting` to the preferred bibliography entry.
\subsection{Initialization}
We crop the RGB target $I^\star$ and foreground mask $M$ to a white
$512\times512$ canvas.  SAM2 masks, frozen DINO features, and smoothed
CIE--Lab colours drive a reversible split tree.  A proposed split is kept
only when all children are connected and hole-free and the local proposal,
semantic, and colour evidence is sufficient.  Bilateral inputs are split on
one canonical half and reflected exactly; a central self-reflected face is
allowed, while the two lateral faces remain separate.  The final faces are
denoted by $\{\Omega_r\}_{r=1}^R$.

Each interface is a shared cubic Bézier chain,
\begin{equation}
 \begin{aligned}
 B_e(t)&=\sum_{j=0}^3b_j(t)q_{e,j},\\
 b_j(t)&=\binom{3}{j}(1-t)^{3-j}t^j,\quad j=0,\ldots,3,
 \end{aligned}
 \label{eq:bezier-boundary}
\end{equation}
where $q_{e,j}\in\mathbb R^2$ are control points.  Interior vertices and
handles are shared across adjacent faces; the exterior contour and true
junctions are fixed.  A bounded $\tanh$ displacement limits every trainable
control motion to four source pixels and preserves topology.

Pins are uniformly sampled in boundary arc length.  For a coloured-string
budget $K$, the default spacing is
\begin{equation}
 \Delta_p=26\sqrt{512/K}\ \text{pixels},
 \label{eq:pin-spacing}
\end{equation}
and junction/silhouette samples are merged.  Each pin $p_i$ stores its
incident faces; bilateral mode also stores a mirror index $\bar i$, so the
two sides share trainable parameters.  A differentiable pin phase uses the
bounded offset $\delta_i=\Delta_i\tanh z_i$.

For each face and local color layer, all distinct incident pin pairs form
$\mathcal C_{r\ell}$.  A pair is legal when its segment lies in a one-pixel
buffer of $\Omega_r$ and is at least eight pixels long; this test is refreshed
after every boundary update.  In the physical Hough chart, a chord with
midpoint $m$, unit normal $n$, and region centre $c_r$ is represented by
\begin{equation}
 \begin{aligned}
 u&=R_r\phi,\quad \phi=\operatorname{atan2}(n_y,n_x)\bmod\pi,\\
 \rho&=(m-c_r)^\top n,
 \end{aligned}
 \label{eq:hough-chart}
\end{equation}
with $(u+\pi R_r,\rho)\sim(u,-\rho)$.  Thus a generatrix is a segment in
the universal cover and candidate distance is the minimum over translated
and endpoint-exchanged lifts.  Initial segments are fitted to high-scoring
target-colour candidates by weighted farthest-point seeding, Lloyd updates,
and PCA endpoints.  The mixed-curves baseline uses two $+1$ and two $-1$
straight families plus ellipse/focus families, then rescales their spans to
obtain approximately $K$ initially selected strings.

\subsection{Differentiable Rendering}
For chord endpoints $a_i,b_i$ and gate $g_i$, we sample the degree-one Bézier
$x_i(t)=(1-t)a_i+tb_i$ at $S=16$ points and render anisotropic Gaussians.
The tangent and normal standard deviations are
$\sigma_\parallel=\|b_i-a_i\|/(2S)+0.5$ and $\sigma_\perp=w/2$ with
$w=0.45$; every sample has opacity $\alpha_0g_i$ with $\alpha_0=0.96$.
Projection, tile binning, and ordered alpha compositing use the CUDA
Bézier-Splatting implementation~\cite{bezier_splatting}; curved mothers use
the same renderer on sampled polyline pieces.

Let $\alpha_{r\ell}(x)$ be the union alpha for face $r$, layer $\ell$, and
$c_{r\ell}$ its spool colour.  Back-to-front compositing is
\begin{equation}
 \begin{aligned}
 C&\leftarrow\alpha_{r\ell}c_{r\ell}+(1-\alpha_{r\ell})C,\\
 V&\leftarrow(1-\alpha_{r\ell})V+\alpha_{r\ell}e_{k(r,\ell)},
 \end{aligned}\label{eq:alpha-over}
\end{equation}
where $C$ starts at white, $V\in\mathbb R^{C+1}$ contains visible spool
masses, and $e_k$ is one-hot; the last channel is a fixed black outline.
Consequently, later layers remove earlier visible mass at the same pixel, so
occlusion is handled directly by alpha-over compositing.  The outline enters
image/colour losses but has detached endpoints and is excluded from the
coloured-string budget.  Soft Gaussian gates are mixed with detached hard
gates from $0$ after $35\%$ of the iterations to $0.9$ at $90\%$.

\subsection{Objective}
Let $V_k(x)$ and $V_o(x)$ be visible coloured and outline masses,
$A=V_o+\sum_kV_k$, and $c_k\in[0,1]^3$ trainable spool colours.  The rendered
image is
\begin{equation}
 \widehat I=\sum_{k=1}^{C}V_kc_k+(1-A)\mathbf1,
 \label{eq:composite}
\end{equation}
because the outline colour is zero and the substrate is white.  A frozen
target-material mixture provides mask $M_T$ and fractions $q_k$.  The baseline
uses the current-RGB similarity
\begin{equation}
 s_k(x)=\exp\!\left(-\frac{\|c_k-I^\star(x)\|_2^2}{2\sigma_c^2}\right),
 \qquad \sigma_c=0.20,
 \label{eq:similarity}
\end{equation}
and Gaussian blur $G_\sigma$.  With desired coverage $\rho=0.35$,
\begin{equation}
 \mathcal L_{\rm mat}=2.5\mathcal L_{\rm wrong}+\mathcal L_{\rm cov}
 +4\mathcal L_{\rm app}+0.02\mathcal L_{\rm bg}.
 \label{eq:material-loss}
\end{equation}
$\mathcal L_{\rm wrong}$ penalizes target-unsupported visible material and
outline mismatch, with one quarter of the multiscale RGB mismatch added;
$\mathcal L_{\rm app}$ is fixed-mask RGB MS--SSIM and $\mathcal L_{\rm bg}$
is outside-mask coverage.  The correct-colour deficit is
\begin{equation}
 \begin{aligned}
 \mathcal L_{\rm cov}&=\frac1{|\Sigma|}\sum_{\sigma\in\Sigma}\\[-1mm]
 &\quad
 \frac{\left\|\left[\rho G_\sigma(M_Tq)-
 G_\sigma\!\left(M_T\sum_kV_ks_k\right)\right]_+\right\|_1}
 {\rho\|G_\sigma(M_T)\|_1},\\
 &\hspace{20mm}\Sigma=\{2,4,8\}.
 \end{aligned}
 \label{eq:coverage-loss}
\end{equation}
The dynamic palette wrapper replaces this demand with a target-balanced local
floor measured from post-occlusion visibility and calibrated relative to the
best initial palette improvement over white; hidden spools receive no credit.

For soft candidate gates $g_i$, the complete baseline scalar is
\begin{equation}
 \begin{aligned}
 \mathcal L={}&\mathcal L_{\rm mat}+2\mathcal L_{\rm cnt}+0.02\mathcal L_{\rm bin}\\
 &+0.01\mathcal L_{\rm col}+0.01\mathcal L_{\rm evid}\\
 &+0.005\mathcal L_{\rm smooth}+5\!\times\!10^{-5}
 (\mathcal L_{\rm ctrl}+\mathcal L_{\rm pin}),\\
 \mathcal L_{\rm cnt}={}&\left(\frac{\sum_i g_i-K}{K}\right)^2,\qquad
 \mathcal L_{\rm bin}=\frac1K\sum_i g_i(1-g_i).
 \end{aligned}\label{eq:total-loss}
\end{equation}
$\mathcal L_{\rm col}$ anchors learned RGB to the initial palette;
$\mathcal L_{\rm evid}$ rewards Bézier samples supported by the frozen
boundary-evidence field; $\mathcal L_{\rm smooth}$ is the normalized cubic
second-difference penalty; and $\mathcal L_{\rm ctrl},\mathcal L_{\rm pin}$
anchor controls and pin phases.  Count matching is soft; hard counts are used
for checkpoint selection and export.

\subsection{Implementation Details}
Training uses CUDA at $256\times256$ rendering resolution, while geometry is
stored in normalized $512$-pixel coordinates.  Adam learning rates are
$0.01$ for pins, $0.03$ for shared Bézier vertices/handles, $0.005$ for
mother and curved-family parameters, and $0.002$ for spool colours.  The
baseline runs 120 iterations, clips the total gradient norm to five, and uses
seed zero.  Each update checks face validity, pin separation, unchanged
adjacency, and current chord legality.  Invalid geometry is projected or
rolled back by a line search with scales $1,1/2,\ldots,1/256$; moments of
restored coordinates are cleared.

Dynamic palette exchanges and reversible mother edits use the same hard,
post-occlusion objective as training.  Hard evaluations occur every ten
iterations; the best state is restored before export, followed by a fixed-parameter greedy deletion of any whole symmetry-tied mother that improves the
hard score.  Geometry, raster, and mother-field caches are scoped to unchanged
states and therefore affect runtime only.


==> sec/08_llm_usage.tex <==
% 中文：大语言模型使用声明。按CVPR 2027作者指南，使用不编号标题，置于正文之后、参考文献之前，并保持作者匿名。
\section*{LLM Usage Statement}
% 中文：我们使用ChatGPT（OpenAI）和DeepSeek辅助代码撰写、数据整理、中文到英文的文本翻译以及示意图绘制。
% 具体涉及方法实现（第4节）、实验数据整理（第5节）、正文和补充材料的英文文本，以及弦空间表示和方法流程的示意图。
% 这些工具用于辅助开展和呈现研究；作者对研究设计、实验结果及解释，以及全部提交内容的准确性、原创性、可复现性和完整性承担全部责任。
We used ChatGPT and DeepSeek to assist with code drafting, data organization, translation, and the preparation of schematic illustrations. This assistance concerned the method implementation (Sec.~\ref{sec:method}), the organization of experimental data (Sec.~\ref{sec:experiments}), English text throughout the main paper and supplementary material, and schematic illustrations of the chord-space representation and method pipeline. These tools served as aids in developing and presenting the work. The authors retain full responsibility for the research design, experimental results and their interpretation, and the accuracy, originality, reproducibility, and integrity of all submitted content.

